Limitations of Deep Learning for Inverse Problems on Digital Hardware

Deep neural networks have seen tremendous success over the last years. Since the training is performed on digital hardware, in this paper, we analyze what actually can be computed on current hardware platforms modeled as Turing machines, which would lead to inherent restrictions of deep learning. For this, we focus on the class of inverse problems, which, in particular, encompasses any task to reconstruct data from measurements. We prove that finite-dimensional inverse problems are not Banach-Mazur computable for small relaxation parameters. Even more, our results introduce a lower bound on the accuracy that can be obtained algorithmically.

==> images/CompFunc_error_bar.tex <==

\begin{figure}[ht]
    \centering
%\scalebox{0.6}{
\begin{tikzpicture}
\begin{axis}[
    axis lines = left,
    ymin=-0.3, ymax=0.5,
    %xmin=-1, xmax=2,
    %xlabel = \(x\),
    %ylabel = {\(f(x)\)},
    yticklabel=\empty,
    xticklabel=\empty
]
%Below the true signal is defined
\addplot [
    domain=-0.9:1.05, 
    samples=100, 
    color=blue,
]
{x^5 -x^4 - x^3 + x^2 };
\addlegendentry{True Signal}

%Below the computed signal is defined
\addplot [
    domain=-0.9:1.05, 
    samples=100, 
    dotted,
    thick,
]
{x^5 -x^4 - x^3 + x^2 +0.1*x };
\addlegendentry{Computed Signal}

%Below the error tube is defined
\addplot [name path=A,black, dotted, domain=-0.9:1.05, samples=100] {x^5 -x^4 - x^3 + x^2 +0.1*x + 0.1 };
\addplot [name path=B,black, dotted, domain=-0.9:1.05, samples=100] {x^5 -x^4 - x^3 + x^2 +0.1*x - 0.1};
\addplot [black!15] fill between[of=A and B];

%Below the error bar is defined
\addplot[
    color=black,    mark=*, error bars/.cd, y dir=both, y explicit, error bar style={line width=1pt},  error mark options={
      rotate=90, mark size=4pt, line width=1pt}
    ]
    coordinates {
    (0.4,0.12064)  +- (0,0.1)
    %(-0.85,0.2859134375)  +- (0,0.1)
    };
    
\node[anchor=north] (source) at (axis cs:0.2,0.3){computed value};
\node (destination) at (axis cs:0.4,0.12064){};
\draw[->,-{latex[scale=5]}, thick](source)  to[bend left=-30]  (destination);    

\node[anchor=north] (source2) at (axis cs:0.6,-0.1){error bar};
\node (destination2) at (axis cs:0.4,0.05){};
\draw[->,-{latex[scale=5]}, thick](source2)  to[bend left=-30]  (destination2); 

\end{axis}
\end{tikzpicture}
%}


\end{figure}

==> images/neural_network.tex <==
\def\layersep{3.75cm}
\begin{figure}[ht]
    \centering
%\scalebox{0.6}{
\begin{tikzpicture}[shorten >=2pt,draw=black!50, node distance=\layersep]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,draw=black,minimum size=17pt,inner sep=0pt]
    \tikzstyle{input neuron}=[neuron, minimum size=0.85cm];
    %\tikzstyle{output neuron max}=[neuron, fill=red!100];
    %\tikzstyle{output neuron other}=[neuron, fill=red!10];
    \tikzstyle{hidden neuron}=[neuron, minimum size=0.85cm];
    \tikzstyle{annot} = [rectangle, draw, very thick, rounded corners, fill=black!25,]
    \tikzstyle{annot2} = [rectangle, draw, very thick, rounded corners, fill=black!25,inner xsep= 1.5pt]
    %\tikzstyle{image} = [rectangle,text centered]

    % Draw the input layer nodes
    \foreach \name / \y in {1,...,3}
        \node[input neuron] (I-\name) at (0,-\y) {$x_\y$};
    
    % Draw the 1st hidden layer nodes
    \foreach \name / \y in {1,...,4}
        \path[yshift=0.5cm]
            node[hidden neuron] (H-\name) at (\layersep,-\y cm) {$\Phi^{(1)}_\y$};
            
    % Draw the 1st hidden layer post-activation nodes
    \foreach \name / \y in {1,...,4}
        \path[yshift=0.5cm]
           node[hidden neuron] (HA-\name) at (\layersep + \layersep/2,-\y cm) {$\Phi^{(1)}_\y$};

    % Draw the 2nd hidden layer nodes
    \foreach \name / \y in {1,...,6}
        \path[yshift=1.5cm]
            node[hidden neuron] (H2-\name) at (2*\layersep + \layersep/2,-\y cm) {$\Phi^{(2)}_\y$};
            
    % Draw the 2nd hidden layer post-activation nodes
    \foreach \name / \y in {1,...,6}
        \path[yshift=1.5cm]
            node[hidden neuron] (HA2-\name) at (3*\layersep,-\y cm) {$\Phi^{(2)}_\y$};

    % Draw the output layer node
    \foreach \name / \y in {1}
        \path[yshift=-1cm]
            node[hidden neuron] (O-\name) at (4*\layersep,-\y cm) {$\Phi$};




    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,...,3}
        \foreach \dest in {1,...,4}
            \path (I-\source) edge[->] (H-\dest);

    % Connect every node in the post activation hidden layer with the second hidden layer
    \foreach \source in {1,...,4}
        \foreach \dest in {1,...,6}
           \path (HA-\source) edge[->] (H2-\dest);

    % Connect every node in the 2nd post-activation hidden layer with the output layer
    \foreach \source in {1,...,6}
        \foreach \dest in {1}
            \path (HA2-\source) edge[->] (O-\dest);
        
    % Connect nodes in the hidden layer with node in the post-activation hidden layer
    \foreach \source in {1,...,4}
        \path (H-\source) edge[->] (HA-\source);
        
    \foreach \source in {1,...,6}
        \path (H2-\source) edge[->] (HA2-\source);
        
    \node[annot, yshift=0.5cm](rho) at (\layersep + \layersep/4,-2.5 cm) {\large $\rho$};
    \node[annot, yshift=0.5cm](rho2) at (2*\layersep + 3*\layersep/4,-2.5 cm) {\large $\rho$};
    
    \node[annot2, yshift=0.5cm](W) at (\layersep/2,-2.5 cm) {$x \mapsto W_1 x + b_1$};
    \node[annot2, yshift=0.5cm](W2) at (2*\layersep,-2.5 cm) {$x \mapsto W_2 x + b_2$};
    \node[annot2, yshift=0.5cm](W3) at (3.5*\layersep,-2.5 cm) {$x \mapsto W_3 x + b_3$};

\end{tikzpicture}
%}


\end{figure}
